BioTool: A Comprehensive Tool-Calling Dataset for Enhancing Biomedical Capabilities of Large Language Models

Despite the success of large language models (LLMs) on general-purpose tasks, their performance in highly specialized domains such as biomedicine remains unsatisfactory. A key limitation is the inability of LLMs to effectively leverage biomedical tools, which clinical experts and biomedical researchers rely on extensively in daily workflows. While recent general-domain tool-calling datasets have substantially improved the capabilities of LLM agents, existing efforts in the biomedical domain largely rely on in-context learning and restrict models to a small set of tools. To address this gap, we introduce BioTool, a comprehensive biomedical tool-calling dataset designed for fine-tuning LLMs. BioTool comprises 34 frequently used tools collected from the NCBI, Ensembl, and UniProt databases, along with 7,040 high-quality, human-verified query-API call pairs spanning variation, genomics, proteomics, evolution, and general biology. Fine-tuning a 4-billion-parameter LLM on BioTool yields substantial improvements in biomedical tool-calling performance, outperforming cutting-edge commercial LLMs such as GPT-5.1. Furthermore, human expert evaluations demonstrate that integrating a BioTool-fine-tuned tool caller significantly improves downstream answer quality compared to the same LLM without tool usage, highlighting the effectiveness of BioTool in enhancing the biomedical capabilities of LLMs. The full dataset and evaluation code are available at https://github.com/gxx27/BioTool

==> backup/backup.tex <==
% \vspace{0.6em}
% \noindent\textbf{Document Context}\par
% \small
% \textit{Description:}
% The search endpoint uses a request query to return all entries associated with the search term in a paginated list of entries.

% \vspace{0.4em}
% \begin{tabularx}{\linewidth}{@{}>{\bfseries}l @{\hspace{0.6em}} X@{}}
% Parameters: &
% \texttt{\footnotesize
% \{ "query": "Criteria to search human diseases (supports AND, OR, NOT)",
%   "sort": "Specify field by which to sort results",
%   "fields": "List of entry sections to return",
%   "size": "Number of entries per page (default: 25, max: 500)" \}}
%\end{tabularx}



% \begin{datacollection}{\small Example of BioTool Data Entry}
%     \noindent\textbf{User Query:} \\
%     Could you provide concise definitions for the major severe immunodeficiency disorders? 
    
%     \vspace{1em}
%     \noindent\textbf{Tool calling Logic:}
%     \begin{itemize}[leftmargin=1.5em, noitemsep, topsep=2pt]
%         \item \textbf{Database:} UniProt
%         \item \textbf{Tool:} \texttt{human\_diseases}
%         \item \textbf{API Endpoint:} \texttt{search\_human\_diseases}
%     \end{itemize}
%     \vspace{1em}
%     \noindent\textbf{API Arguments:}
%     \begin{itemize}[leftmargin=1.5em, noitemsep, topsep=2pt]
%         \item \textbf{"query":} \texttt{"name:immunodeficiency AND name:severe"}
%         \item \textbf{"fields":} \texttt{"definition"}
%         \item \textbf{"sort":} \texttt{"id asc"}
%     \end{itemize}
%     \vspace{1em}
%     % \noindent\textbf{Observation:} \\
%     % \texttt{\small\{'results': [\{'id': 'DI-00171', 'definition': 'An autosomal recessive immunologic disorder characterized by the loss of expression of MHC class II antigens on antigen-presenting cells. Affected individuals present in early infancy with severe recurrent bacterial, viral, fungal and parasitic infections, usually affecting the gastrointestinal and respiratory tracts.'\}, \{'id': 'DI-00304', 'definition': 'A form of chronic granulomatous disease, a primary immunodeficiency characterized by severe recurrent bacterial and fungal infections, along with manifestations of chronic granulomatous inflammation. It results from an impaired ability of phagocytes to mount a burst of reactive oxygen species in response to pathogens.'\}, \{'id': 'DI-00305', 'definition': 'A form of chronic granulomatous disease, a primary immunodeficiency characterized by severe recurrent bacterial and fungal infections, along with manifestations of chronic granulomatous inflammation. It results from an impaired ability of phagocytes to mount a burst of reactive oxygen species in response to pathogens.', ...\}]\}}
%     % \vspace{1.5em}
%     % \noindent\textbf{Document Context:} \\
%     % \textit{Description:} The search endpoint uses a request query to return all entries associated with the search term in a paginated list of entries.
%     % \vspace{0.5em}
%     % \texttt{\footnotesize "\{"parameters": \{"type": "object", "properties": \{"query": \{"type": "string", "description": "Criteria to search human diseases. Advanced queries can be built with parentheses and conditionals such as AND, OR and NOT."\}, "sort": \{"type": "string", "description": "Specify field by which to sort results."\}, "fields": \{"type": "string", "description": "List of entry sections (fields) to be returned, separated by commas."\}, "size": \{"type": "integer", "description": "Specify the number of entries per page of results (Pagination size). Default is 25, max is 500"\}\}, "additionalProperties": false, "required": ["query"]\}\}"}
% \end{datacollection}

% \newtcolorbox{datacollection}[1]{
%     breakable,
%     colback=white,
%     colframe=gray!20,
%     colbacktitle=gray!10,
%     coltitle=black,
%     fonttitle=\bfseries\sffamily,
%     title=#1,
%     sharp corners,
%     boxrule=0.5pt,
%     left=3mm,
%     right=3mm,
%     top=3mm,
%     bottom=3mm,
%     middle=2mm,
%     width=\columnwidth,
%     fontupper=\rmfamily\small,
%     before skip=12pt,
%     after skip=12pt
% }

% \begin{table*}
% \centering
% % \small
% \begin{tabular}{lcccccccc}
% \toprule
% \textbf{Model} & \multicolumn{2}{c}{\textbf{NCBI}} & \multicolumn{2}{c}{\textbf{UniProt}} & \multicolumn{2}{c}{\textbf{Ensembl}} & \multicolumn{2}{c}{\textbf{Overall (Avg)}} \\
% & CS & AS & CS & AS & CS & AS & CS & AS \\
% \midrule
% \textit{Proprietary Models} & & & & & & & & \\
% GPT-5.1 & 0.1214 & 0.1660 & 0.5279 & 0.9788 & 0.6296 & 0.7939 & 0.4238 & 0.6435 \\
% GPT-5.1 Codex & 0.1096 & 0.1618 & 0.5707 & 0.9830 & 0.6619 & 0.8048 & 0.4447 & 0.6470 \\
% Gemini 3 Pro & 0.5395 & 0.8004 & 0.4499 & 0.8832 & 0.4339 & 0.8308 & 0.4749 & 0.8381 \\
% Claude 4.5 Sonnet & 0.7639 & 0.8550 & 0.7030 & \textbf{1.0000} & 0.7015 & 0.8243 & 0.7231 & 0.8935 \\
% \midrule
% \textit{Fine-tuned Open-Source} & & & & & & & & \\
% GPT-OSS-20B (LoRA) & 0.8559 & 0.9454 & 0.5697 & 0.9851 & 0.7988 & 0.9262 & 0.7415 & 0.9524 \\
% Llama 3.1-8B-Instruct (LoRA) & 0.9002 & 0.9433 & 0.7686 & 0.9979 & 0.8864 & 0.9588 & 0.8517 & 0.9666 \\
% Qwen 3-8B (LoRA) & 0.8837 & 0.9349 & 0.6787 & 0.9958 & 0.7570 & 0.8590 & 0.7736 & 0.9304 \\
% Qwen 2.5-7B-Instruct (LoRA) & 0.9053 & 0.9391 & 0.7463 & \textbf{1.0000} & 0.8116 & 0.8785 & 0.8214 & 0.9396 \\
% Qwen 3-4B-Instruct & \textbf{0.9268} & \textbf{0.9454} & \textbf{0.8106} & 0.9979 & \textbf{0.9286} & \textbf{0.9805} & \textbf{0.8885} & \textbf{0.9744} \\
% \bottomrule
% \end{tabular}
% \caption{Performance comparison of proprietary and open-source models on the BioTool-Bench dataset (1,408 samples). CS denotes the Complete Score and AS denotes API Success. Open-source models were fine-tuned using LoRA on our curated biomedical dataset, while Qwen 3 4B shows exceptional zero-shot/specialized capability.}
% \label{tab:results}
% \end{table*}

% \begin{table*}
% \centering
% \begin{tabular}{lcccccccc}
% \toprule
% \textbf{Model} & \multicolumn{2}{c}{\textbf{NCBI}} & \multicolumn{2}{c}{\textbf{UniProt}} & \multicolumn{2}{c}{\textbf{Ensembl}} & \multicolumn{2}{c}{\textbf{Overall (Avg)}} \\
% & CS & AS & CS & AS & CS & AS & CS & AS \\
% \midrule
% \textit{Proprietary Models} & & & & & & & & \\
% GPT-5.1 & 0.121 & 0.166 & 0.528 & 0.979 & 0.630 & 0.794 & 0.424 & 0.644 \\
% GPT-5.1-Codex & 0.110 & 0.162 & 0.571 & 0.983 & 0.662 & 0.805 & 0.445 & 0.647 \\
% Gemini 3 Pro & 0.540 & 0.800 & 0.450 & 0.883 & 0.434 & 0.831 & 0.475 & 0.838 \\
% Claude 4.5 Sonnet & 0.764 & 0.855 & 0.703 & \textbf{1.000} & 0.702 & 0.824 & 0.723 & 0.894 \\
% \midrule
% \textit{Fine-tuned Open Source} & & & & & & & & \\
% gpt-oss-20b (LoRA) & 0.856 & 0.945 & 0.570 & 0.985 & 0.799 & 0.926 & 0.742 & 0.952 \\
% Llama3.1-8B-Instruct (LoRA) & 0.900 & 0.943 & 0.769 & 0.998 & 0.886 & 0.959 & 0.852 & 0.967 \\
% Qwen3-8B (LoRA) & 0.884 & 0.935 & 0.679 & 0.996 & 0.757 & 0.859 & 0.774 & 0.930 \\
% Qwen2.5-7B-Instruct (LoRA) & 0.905 & 0.939 & 0.746 & \textbf{1.000} & 0.812 & 0.879 & 0.821 & 0.940 \\
% Qwen3-4B-Instruct & \textbf{0.927} & \textbf{0.945} & \textbf{0.811} & 0.998 & \textbf{0.929} & \textbf{0.981} & \textbf{0.889} & \textbf{0.974} \\
% \bottomrule
% \end{tabular}
% \caption{Comparative evaluation of proprietary and open source models across the three primary database subsets of the \textsc{BioTool} dataset. The metrics include the Complete Score, denoted as CS, and API Success, denoted as AS. Open source models were fine-tuned using LoRA on the \textsc{BioTool} training set to acquire specialized domain knowledge, while proprietary models were evaluated under standard inference conditions.}
% \label{tab:results}
% \end{table*}

\paragraph{Complete Score (CS)} 
The \textsc{CS} serves as our primary composite metric, evaluating the alignment of retrieved information with the user's intent by synthesizing the technical precision of \textsc{EM} and the functional reliability of \textsc{AS}:

$$CS = EM + (1 - EM) \cdot AS \cdot \text{similarity}(O_{gen}, O_{ref})$$

where $O_{gen}$ represents the biological observation retrieved from the live API based on the model's call, and $O_{ref}$ denotes the definitive reference observation stored in our dataset. This formulation is specifically designed for the biomedical domain: an exact match ($EM=1$) ensures a correct response ($CS=1.0$), while an API failure ($AS=0$) indicates the model cannot retrieve necessary data, leading to untrustworthy hallucinations ($CS=0.0$). For successful calls that do not match the reference exactly ($AS=1, EM=0$),  We therefore utilize semantic similarity, which is calculated through text embedding similarity, to assess the difference between $O_{gen}$ and $O_{ref}$. 

\paragraph{API Success (AS)} 
The \textsc{AS} metric tracks the syntactic and logical validity of the model's output. A generated call is considered successful ($AS=1$) if it executes correctly and returns a valid response containing data. Conversely, if the call fails due to incorrect formatting, invalid API names, or improper parameter values, it is recorded as a failure ($AS=0$).


\paragraph{Exact Match (EM)} 
\textsc{EM} measures whether the generated API call is identical to the ground-truth reference, representing the highest level of technical precision. For a sample to be considered an exact match ($EM=1$), the model must correctly identify the API name and provide all required parameters with values matching the reference exactly.


% This is the original version
% \begin{table}[t]
% \centering
% \setlength{\tabcolsep}{2pt}

% \begin{tabular}{lcccc}
% \toprule
% {\textbf{Model}} &
% {\small\textbf{NCBI}} &
% {\small\textbf{UniProt}} &
% {\small\textbf{Ensembl}} &
% {\small\textbf{Overall}} \\
% \midrule

% \rowcolor{gray!15}
% \multicolumn{5}{c}{\small{Proprietary Models}}\vspace{0.1cm} \\
% GPT-5.1 & 12.1 & 52.8 & 63.0 & 42.4 \\
% GPT-5.1-Codex & 11.0 & 57.1 & 66.2 & 44.5 \\
% Gemini 3 Pro & 68.0 & 72.1 & 71.2 & 70.4 \\
% Claude 4.5 Sonnet & 76.4 & 70.3 & 70.2 & 72.3 \\

% \midrule
% \rowcolor{gray!15}
% \multicolumn{5}{c}{\small{BioTool Finetuned Open Source Models}}\vspace{0.1cm} \\

% gpt-oss-20b & 85.6 & 57.0 & 79.9 & 74.2 \\
% Llama3.1-8B-Ins & 90.0 & 76.9 & 88.6 & 85.2 \\
% Qwen3-8B & 88.4 & 67.9 & 75.7 & 77.4 \\
% Qwen2.5-7B-Ins & 90.5 & 74.6 & 81.2 & 82.1 \\
% Qwen3-4B-Ins & \textbf{92.7} & \textbf{81.1} & \textbf{92.9} & \textbf{88.9} \\

% \bottomrule
% \end{tabular}

% \caption{Comparative evaluation of models based on the Complete Score (CS) across the \textsc{BioTool} dataset subsets. Higher CS indicates better performance; bold values denote the best results in each column.}
% \label{tab:results_cs}
% \end{table}

% \begin{table*}[t]
% \centering
% \begin{tabular}{lcccc}
% \toprule
% \textbf{Model} & \textbf{NCBI} & \textbf{UniProt} & \textbf{Ensembl} & \textbf{Overall} \\
% \midrule
% \textit{Proprietary Models} & & & & \\
% GPT-5.1 & 0.121 & 0.528 & 0.630 & 0.424 \\
% GPT-5.1-Codex & 0.110 & 0.571 & 0.662 & 0.445 \\
% Gemini 3 Pro & 0.680 & 0.721 & 0.712 & 0.704 \\
% Claude 4.5 Sonnet & 0.764 & 0.703 & 0.702 & 0.723 \\
% \midrule
% \textit{BioTool Finetuned} & & & & \\
% gpt-oss-20b & 0.856 & 0.570 & 0.799 & 0.742 \\
% Llama3.1-8B-Instruct & 0.900 & 0.769 & 0.886 & 0.852 \\
% Qwen3-8B & 0.884 & 0.679 & 0.757 & 0.774 \\
% Qwen2.5-7B-Instruct & 0.905 & 0.746 & 0.812 & 0.821 \\
% Qwen3-4B-Instruct & \textbf{0.927} & \textbf{0.811} & \textbf{0.929} & \textbf{0.889} \\
% \bottomrule
% \end{tabular}
% \caption{Comparative evaluation of models based on the Complete Score (CS) across the \textsc{BioTool} dataset subsets. Higher CS indicates better performance; bold values denote the best results in each column.}
% \label{tab:results_cs}
% \end{table*}


% \begin{table*}[t]
% \centering
% \begin{tabular}{lcccccccc}
% \toprule
% \textbf{Model} & \multicolumn{2}{c}{\textbf{NCBI}} & \multicolumn{2}{c}{\textbf{UniProt}} & \multicolumn{2}{c}{\textbf{Ensembl}} & \multicolumn{2}{c}{\textbf{Overall (Avg)}} \\
% & EM & AS & EM & AS & EM & AS & EM & AS \\
% \midrule
% \textit{Proprietary Models} & & & & & & & & \\
% GPT-5.1 & 0.000 & 0.166 & 0.017 & 0.979 & 0.089 & 0.794 & 0.035 & 0.644 \\
% GPT-5.1-Codex & 0.000 & 0.162 & 0.017 & 0.983 & 0.063 & 0.805 & 0.026 & 0.647 \\
% Gemini 3 Pro & 0.032 & 0.767 & 0.021 & 0.998 & 0.163 & 0.820 & 0.071 & 0.862 \\
% Claude 4.5 Sonnet & 0.036 & 0.855 & 0.011 & \textbf{1.000} & 0.150 & 0.824 & 0.065 & 0.894 \\
% \midrule
% \textit{Fine-tuned Open Source} & & & & & & & & \\
% gpt-oss-20b (LoRA) & 0.307 & 0.945 & 0.040 & 0.985 & 0.304 & 0.926 & 0.217 & 0.952 \\
% Llama3.1-8B-Instruct (LoRA) & 0.422 & 0.943 & 0.072 & 0.998 & 0.430 & 0.959 & 0.308 & 0.967 \\
% Qwen3-8B (LoRA) & 0.437 & 0.935 & 0.040 & 0.996 & 0.377 & 0.859 & 0.285 & 0.930 \\
% Qwen2.5-7B-Instruct (LoRA) & 0.456 & 0.939 & 0.055 & \textbf{1.000} & 0.423 & 0.879 & 0.311 & 0.940 \\
% Qwen3-4B-Instruct & \textbf{0.656} & \textbf{0.945} & \textbf{0.093} & 0.998 & \textbf{0.518} & \textbf{0.981} & \textbf{0.423} & \textbf{0.974} \\
% \bottomrule
% \end{tabular}
% \caption{Comparative evaluation of Exact Match (EM) and API Success (AS) metrics. Higher EM indicates better structural adherence to documentation, while higher AS indicates functional validity. Bold values denote the best results in each column.}
% \label{tab:results_em_as}
% \end{table*}

%Second, the performance across the different database subsets indicates that fine-tuned models are more adept at internalizing the heterogeneous logic required by distinct biological APIs. On the NCBI subset, which often requires complex parameter configurations, the fine-tuned models achieved a performance margin of nearly 12.4\% over the proprietary baselines. While proprietary models often struggle to bridge the gap between natural language queries and the rigid, often non-intuitive requirements of live biological endpoints, the fine-tuned models demonstrate a superior ability to align user intent with the specific data structures of the underlying repositories. These findings suggest that the path toward reliable biomedical agents relies less on increasing model size and more on the utilization of human-verified, scientifically rigorous data to refine model reasoning within the target domain.

%As biological APIs return highly diverse content without a fixed format across different database endpoints, simple literal string matching is often insufficient.

%To provide a comprehensive assessment of model performance, we introduce three primary metrics that evaluate distinct aspects of the tool-calling process: structural precision, execution reliability, and semantic correctness.

%The primary factor in a model's usefulness is the actual quality of its answers. To evaluate this, we performed a human assessment on 700 samples randomly drawn from the BioTool test set. Two researchers with at least a college-level background in bioinformatics did manual side-by-side comparisons of the responses. The evaluators were instructed to select the superior answer based on its informativeness and how effectively it fulfilled the user's specific request, while rejecting responses that were vague or scientifically incorrect. We compared three distinct configurations: a base GPT-5.1 model responding without any tool access (None), a version provided with ground-truth biological observations from our dataset (Oracle), and a version utilizing tool calls generated by our fine-tuned Qwen3-4B-Instruct model (Qwen3-4B). 

%samples divided almost evenly among the three foundational repositories, which prevents models from developing technical biases toward any single database schema or implementation style. Beyond source distribution, the dataset is characterized by its broad functional utility and extensive biological domain coverage. As shown in Figure~\ref{fig:statistics}(b), the API categories support diverse functional workflows, ranging from data retrieval (46.0\%) for fetching specific records such as protein sequences or nucleotide identifiers, to search and discovery (41.0\%) for navigating datasets via keywords or phenotypes. More technically intensive analysis and mapping (12.2\%) tasks are also represented, including cross-referencing SNP identifiers to genomic coordinates and performing sequence similarity searches. In tandem, the biological domain distribution in Figure~\ref{fig:statistics}(c) highlights the dataset's extensive scientific scope. While grounded in genomics (40.8\%), encompassing tasks such as searching gene trees, fetching full genomic sequences, and analyzing transcript structures, and proteomics (28.2\%) for protein annotations and complex sequence alignments, the dataset provides significant depth in other specialized areas. The variation (15.1\%) domain focuses on retrieving clinical variants and assessing their functional impacts through tools like the Variant Effect Predictor or analyzing linkage disequilibrium. Furthermore, representation in literature (7.2\%) for citation searches and evolutionary biology (6.3\%) for taxonomy and species-level identification ensures that models acquire the necessary context for both broad and niche research scenarios. This comprehensive coverage is further reflected in the tool usage distribution in Figure~\ref{fig:statistics}(d), which balances frequently accessed general utilities with a long tail of specialized tools. This distribution provides the robust training signal required for models to assist in intricate scientific discovery across the entire central dogma.

% This metric serves as the baseline for determining whether a model can interact with professional biological tools in a technically accurate manner.

% \begin{figure*}[t]
%     \centering
%     \includegraphics[width=\textwidth]{figs/stats.png}
%     \caption{Distribution analysis of the 7,040 samples within \textsc{BioTool} across three dimensions. Panel (a) shows the distribution across source databases. Panel (b) illustrates the functional classification of the API calls. Panel (c) highlights the coverage of diverse biological domains.}
%     \label{fig:statistics}
% \end{figure*}

% \begin{figure*}[t]
%     \centering
%     \includegraphics[width=\textwidth]{figs/tool_usage.png}
%     \caption{The distribution of the total number of user queries generated for each distinct biological tool utilized in the dataset.}
%     \label{fig:tool_usage}
% \end{figure*}


%For each successful API interaction, we utilized the OpenAI o3 model~\cite{openai2025o3o4mini} to generate two distinct natural language User Queries, resulting in an initial pool of 12,782 queries and API pairs. The generation process follows a Chain-of-Thought two-phase reasoning strategy designed to simulate the specific requirements of a biomedical researcher~\cite{wei2023chainofthoughtpromptingelicitsreasoning}. During the first phase, the model performs parameter mapping and abstraction to translate technical data into natural language concepts. This involves keeping unique identifiers verbatim while mapping numerical thresholds to qualitative adjectives such as significant or conserved. The second phase produces two specific types of questions: a broad implicit query that a researcher might ask a colleague and a qualitative query that targets a specific feature of the data. This strategy ensures a condition of \textit{necessity}, where the parameters and functions of the tool are essential to satisfying the user intent without the query explicitly naming the tool. This grounding prevents the creation of generic questions and ensures that the API is the logical choice for an answer. 

%Following the generation of queries, we implemented an LLM-as-a-Judge framework~\cite{zheng2023judgingllmasajudgemtbenchchatbot} leveraging Claude Haiku 4.5~\cite{anthropic2025haiku45} to perform an informative check on the resulting query-observation pairs. The primary goal of this validator is to establish \textit{Sufficiency} by determining whether the provided API observation contains enough information to answer the user query. This step is critical to mitigate hallucinations where the generated question might ask for details that the retrieved data does not actually contain. The model follows a rubric that classifies a pair as informative if the observation contains at least one relevant fact or a partial summary that supports the user intent. We discard any pairs where the observation content is unrelated to the query or too vague to support a concrete response. By focusing on the alignment between the question and the retrieved data, this process ensures that every entry in the final dataset contains a verifiable biological observation that satisfies the query. 
